Detection and Mitigation of Rare Subclasses in Deep Neural Network Classifiers

Regions of high-dimensional input spaces that are underrepresented in training datasets reduce machine-learnt classifier performance, and may lead to corner cases and unwanted bias for classifiers used in decision making systems. When these regions belong to otherwise well-represented classes, their presence and negative impact are very hard to identify. We propose an approach for the detection and mitigation of such rare subclasses in deep neural network classifiers. The new approach is underpinned by an easy-to-compute commonality metric that supports the detection of rare subclasses, and comprises methods for reducing the impact of these subclasses during both model training and model exploitation. We demonstrate our approach using two well-known datasets, MNIST's handwritten digits and Kaggle's cats/dogs, identifying rare subclasses and producing models which compensate for subclass rarity. In addition we demonstrate how our run-time approach increases the ability of users to identify samples likely to be misclassified at run-time.

==> sections/CorrectCatsTable.tex <==
\setlength\tabcolsep{1.5pt} 
\begin{tabular}{ccccc}
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img0.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img1.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img2.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img3.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img4.png} \\
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img5.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img6.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img7.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img8.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img9.png} \\
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img10.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img11.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img12.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img13.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img14.png} \\
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img15.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img16.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img17.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img18.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img19.png} \\
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img20.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img21.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img22.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img23.png} &
	\includegraphics[scale=0.50]{images/Misclassification/MCOnly/CorrectCats/MCCats-img24.png} 
\end{tabular}	


==> sections/UnlabelledTable.tex <==
\clearpage
\onecolumn
%\section{Samples identified at run-time\label{sec:run-time-samples}}
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{2pt}%
%\setlength\tabcolsep{1.5pt}
\renewcommand*{\arraystretch}{0.8}
\begin{longtable}{cccccccccc}
\caption{Samples identified at run-time as having a low commonality score. The labels underneath the images indicates the model prediction. Misclassified images are highlighted with a red border and an asterix on the predicted label.\label{tab:runTimeSamples}}\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2308.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1897.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/12475.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/12203.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/6147.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4523.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/7499.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1358.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1852.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10672.jpg}\\
	dog&cat&cat&cat&cat&cat&cat *&dog&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/91.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5230.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7673.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5702.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4721.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2961.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11324.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9348.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/12058.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/9558.jpg}}\\
	cat&cat&cat&cat&cat&dog&cat&cat&cat&cat *\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3987.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3560.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/7107.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10856.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9459.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/150.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3995.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7707.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5205.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/11058.jpg}}\\
	dog&cat&cat *&cat&cat&cat&cat&dog&cat&dog *\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5604.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/9822.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/12110.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1506.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7773.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/10772.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2013.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8687.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2433.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5826.jpg}\\
	dog&cat *&cat&dog&cat&cat *&cat&cat&dog&dog\\
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/4747.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8168.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10959.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/734.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2294.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/676.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4644.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10012.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10637.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/6434.jpg}\\
	cat *&cat&dog&cat&dog&cat *&cat&cat&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4949.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8183.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4728.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/3573.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11813.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/12166.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/8630.jpg}}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/3159.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10402.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2970.jpg}\\
	cat&dog&cat&dog *&cat&cat&cat *&cat *&cat&cat\\
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/4801.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10908.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/6301.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3170.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1475.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/5978.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7571.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2369.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/444.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7749.jpg}\\
	cat *&cat&dog&dog&cat&dog *&cat&cat&cat&cat\\
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/8814.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/509.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10303.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3930.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/7270.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4583.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11132.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/237.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9638.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11318.jpg}\\
	dog *&dog&cat&cat&dog *&cat&dog&cat&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7303.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4753.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8279.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/8731.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4910.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8282.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4519.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/12289.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11460.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4322.jpg}\\
	cat&cat&dog&cat *&cat&cat&cat&dog&cat&dog\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1255.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8959.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/5013.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3776.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4522.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/1605.jpg}}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/11181.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3465.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8443.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/234.jpg}\\
	cat&dog&dog *&cat&cat&cat *&cat *&cat&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9012.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8044.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11353.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10840.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5777.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/7129.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7570.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4848.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5564.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/595.jpg}\\
	cat&cat&cat&cat&dog&cat *&cat&cat&cat&dog\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8618.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2242.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4326.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/4132.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9422.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2805.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/331.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2408.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5202.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2496.jpg}\\
	cat&cat&cat&cat *&cat&cat&cat&cat&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7983.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3502.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8625.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/838.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7317.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3562.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8899.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9365.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1163.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1204.jpg}\\
	cat&cat&cat&cat&cat&dog&cat&dog&cat&cat\\
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/5471.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5267.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8425.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7893.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2535.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/1458.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11743.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10073.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/6445.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3172.jpg}\\
	cat *&cat&cat&dog&cat&cat *&cat&dog&cat *&cat\\
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/7713.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/84.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/7943.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3313.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/409.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/290.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/193.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/782.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7968.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3207.jpg}\\
	cat *&cat&dog *&cat&cat&cat&cat&cat&cat&cat\\
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/536.jpg}}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/6293.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/191.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10489.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2137.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8580.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1466.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2044.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7432.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/392.jpg}}\\
	cat *&cat *&cat&cat&cat&cat&cat&cat&cat&cat *\\
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/4785.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10843.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/12449.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2278.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2153.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1808.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11345.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/426.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4687.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1689.jpg}\\
	dog *&cat&cat&cat&cat&cat&cat&cat&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9979.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11456.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8858.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7262.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2051.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8125.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5856.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11194.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11483.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/6334.jpg}\\
	cat&cat&cat&cat&cat&cat&cat&dog&dog&cat\\
		\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/6964.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1117.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/524.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7512.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/2094.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3228.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2335.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9897.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11724.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/6695.jpg}\\
	dog *&cat&cat&cat&dog *&cat&cat&cat&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/12439.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1889.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/124.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/4860.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5506.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8587.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4293.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9836.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/8859.jpg}}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/641.jpg}}\\
	dog&cat&cat&cat *&cat&cat&cat&dog&dog *&cat *\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8530.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/6251.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1339.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11240.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9261.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5059.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7156.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9307.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5615.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2553.jpg}\\
	cat&dog *&cat&cat&dog&cat&cat&cat&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9112.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1857.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5927.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/5671.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/4903.jpg}}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/6486.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4296.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11757.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8194.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/12388.jpg}\\
	cat&cat&cat&cat&dog *&dog *&cat&dog&dog&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10229.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/2678.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3388.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11595.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2973.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/6249.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/8783.jpg}}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10471.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1649.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/2542.jpg}\\
	cat&cat *&cat&cat&cat&dog&dog *&cat&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/9559.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/8151.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4682.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4807.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/552.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11685.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3171.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11745.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/514.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/7962.jpg}\\
	dog&cat&cat&cat&dog&cat&cat&cat&cat&cat\\
	\includegraphics[scale=0.15]{images/PGF/unlabelled/11634.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1112.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/3265.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/4252.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/10760.jpg}&
	\includegraphics[scale=0.15]{images/PGF/unlabelled/1702.jpg}&
	\fcolorbox{red}{red}{\includegraphics[scale=0.15]{images/PGF/unlabelled/6444.jpg}}& & & \\
	cat & cat & cat & dog & cat & dog & cat * & & & \\
\end{longtable}


==> sections/meta.tex <==
%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below.
%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010257</concept_id>
<concept_desc>Computing methodologies~Machine learning</concept_desc>
<concept_significance>500</concept_significance>
</concept>

</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Machine learning}
%
% End generated code
%




\keywords{Machine learning, rare cases, rare classes, class imbalance, safety-critical systems, assurance, assurance evidence}

==> sections/modelsTable.tex <==

\begin{table*}
    \centering
        \caption{Models used for evaluation}
    \label{tab:EvalModels}
    \begin{tabular}{lcc}
    \toprule
         & MNIST & CatsDogs \\ \midrule
         Training Set Size & 60,000 & 25,000 \\
         Testing Set & 10,000 & 4989\\
         Image Type & Grayscale 28x28 & RGB size varies\\
         Number of Classes & 10 & 2 \\ \midrule
         Model Source &  \href{https://github.com/keras-team/keras/blob/master/examples/mnist_cnn.py}{Keras development team}
         &\href{https://www.kaggle.com/c/dogs-vs-cats/data}{Kaggle competition entry} \\ \midrule
         Layer 1 & Conv(32) & Conv(32), BatchNorm, MaxPool, DropOut \\
         Layer 2 & Conv(64), MaxPool, DropOut & Conv(64), BatchNorm, MaxPool, DropOut \\
         Layer 3 & Dense(128), DropOut & Conv(64), BatchNorm, MaxPool, DropOut \\
         Layer4 & SoftMax(10) &   Dense(512), BatchNorm, DropOut \\
         Layer5 & - & SoftMax(2)\\ \midrule
         Trainable parameters & 1,199,882 & 12,942,786 \\
         Validation acc. & 0.9913 & 0.8953 \\ \bottomrule
    \end{tabular}

\end{table*}


